Joint Channel Estimation and Synchronization Techniques for Time Interleaved Block Windowed Burst OFDM

From a conceptual perspective, 5G technology promises to deliver low latency, high data rate and more reliable connections for the next generations of communication systems. To face these demands, modulation schemes based on Orthogonal Frequency Domain Multiplexing (OFDM) can accommodate these requirements for wireless systems. On the other hand, several hybrid OFDM-based systems such as the Time-Interleaved Block Windowed Burst Orthogonal Frequency Division Multiplexing (TIBWB-OFDM) are capable of achieving even better spectral confinement and power efficiency. This paper addresses to the implementation of the TIBWB-OFDM system in a more realistic and practical wireless link scenarios by addressing the challenges of proper and reliable channel estimation and frame synchronization. We propose to incorporate a preamble formed by optimum correlation training sequences, such as the Zadoff-Chu (ZC) sequences. The added ZC preamble sequence is used to jointly estimate the frame beginning, through signal correlation strategies and a threshold decision device, and acquire the channel state information (CSI), by employing estimators based on the preamble sequence and the transmitted data. The employed receiver estimators show that it is possible to detect the TIBWB-OFDM frame beginning and provide a close BER performance comparatively to the one where the perfect channel is known.

==> Chapter/01_abstract.tex <==
From a conceptual perspective, 5G technology promises to deliver low latency, high data rate and more reliable connections for the next generations of communication systems. To face these demands Orthogonal Frequency Domain Multiplexing (OFDM) systems can accommodate these requirements for wireless systems. On the other hand, several hybrid OFDM-based systems such as the Time-Interleaved Block Windowed Burst Orthogonal Frequency Division Multiplexing (TIBWB-OFDM) are capable of achieving even better spectral confinement and power efficiency.
%
This paper addresses to the implementation of the TIBWB-OFDM system in a more realistic and practical wireless link scenarios by incorporating optimum correlation training sequences, such as the Zadoff-Chu (ZC) sequences, on the block burst transceivers schemes for proper and reliable channel estimation and frame synchronization algorithms in a SISO communication system. 
%
The proposed TIBWB-OFDM transmitted block is now composed by an amplified ZC preamble sequence used to jointly estimate the frame beginning, through signal correlation strategies and a threshold decision device, and acquire the channel state information, by employing estimators based on the preamble sequence and the transmitted data. 
%
The employed receiver system estimators show that it is possible to detect the TIBWB-OFDM frame beginning and provide similar BER performance comparatively to the one where the perfect channel is known.
%The Time Interleave 
%In the segment of communications industry, wireless mobile communications are one of the most important innovations of our times due to its impact in the global economy and society. Expectations grow with the arrival and demands that the fifth generation of mobile telecommunications (5G) brings associated with an everywhere user access with better reliability and quality.
%From a conceptual perspective, 5G technology promises to deliver low latency, high speed and more reliable connections to new generations of autonomous systems and edge-type devices, covering both massive and critical machine-type communications.
%
%In this context, \textit{Orthogonal Frequency Division Multiplexing} (OFDM) is a widely used system that guarantees robustness against frequency selectivity channels, provide high data transmission rates and a easy implementation based on the discrete Fourier transform.
%
%However, this technique has high limited spectral efficiency, low power efficiency and sensitivity to synchronization errors.
%
%As an alternative, hybrid modulation techniques such as the time interleaved block windowed burst orthogonal frequency division multiplexing (\acs{tibwb-ofdm}) were developed.
%

%This thesis develops the \acs{tibwb-ofdm} transceiver model and the modifications necessary to implement this technique in a real wireless link scenarios. Hence, channel estimation and frame synchronization algorithms were the key challenges and focus of this work.
%
%An important step to achieve reliable frame synchronization is the choice of preamble sequences with optimum correlation proprieties, such as the Zadoff-Chu (\acs{zc}) sequences. 
%
%Our experimental results show that by applying a correlation algorithm and a threshold device it is possible to detect perfectly each \acs{tibwb-ofdm} frame beginning. On the other hand, \acs{zc} sequences were also used to acquire the channel information by applying estimators and algorithms based on the \acs{ofdm} technique.

%Therefore, this thesis proposes a joint channel and frame synchronization estimation using power amplified \acs{zc} sequences as preambles in the \acs{tibwb-ofdm} method.\\
